Extremes of the 2d scale-inhomogeneous discrete Gaussian free field: Convergence of the maximum in the regime of weak correlations

We continue the study of the maximum of the scale-inhomogeneous discrete Gaussian free field in dimension two. In this paper, we consider the regime of weak correlations and prove the convergence in law of the centred maximum to a randomly shifted Gumbel distribution. In particular, we obtain limiting expressions for the random shift. As in the case of variable speed branching Brownian motion, the shift is of the form CY, where C is a constant that depends only on the variance at the shortest scales, and Y is a random variable that depends only on the variance at the largest scales. Moreover, we investigate the geometry of highest local maxima. We show that they occur in clusters of finite size that are separated by macroscopic distances. The poofs are based on Gaussian comparison with branching random walks and second moment estimates.

==> approximation_general_field.tex <==
We want point out that we can actually generalize our approach to more general covariance functions. In particular, we can drop the assumption of finitely many scales. In the following, we remark on what has to be altered in the proof. Key ingredients in the prove of convergence in law is that we can define an approximating field $S^N_v$ satisfying covariance approximations as stated in ... . The other key that one needs precise right-tail asymptotics for the field.
In general, we have $\psi^N_v=\int_{0}^{1}\sigma(s)\nabla \phi^N_v(s)\mathrm{d}s,$ and assume that $\mathcal{I}_{\sigma^2}(1)=1$ and that, for $x\in (0,1)$, $\mathcal{I}_{\sigma^2}(x)<x$. Furthermore, we want that $s\mapsto \sigma(s)$ has bounded first derivative.
We make the following ansatz:
\begin{align}\label{equation:ansatz}
	\psi^N_v= \int_{0}^{\epsilon}\sigma(s)\nabla \phi^N_v(s) \mathrm{d}s + \int_{\epsilon}^{1-\epsilon} \sigma(s)\nabla \phi^N_v(s) \mathrm{d}s + \int_{1- \epsilon}^{1}\sigma(s)\nabla \phi^N_v(s)\mathrm{d}s.
\end{align}
For the first and third summand, we want to use, in principle, the same approximation as in the case of finitely many scales.
For the second term, we want to simply use a MIBRW approximation, precisely as in .
To justify  this choice, we note that by a simple Taylor expansion,
\begin{align}\label{equation:1}
	\sigma(s)=\sigma(0)+\sigma^\prime(0)s+ O(s), \, s\in [0,\epsilon]
\end{align}
and
\begin{align}\label{equation:2}
	\sigma(s)=\sigma(1)+\sigma^\prime(1)(s-1) + O((s-1)),\, s\in [1-\epsilon,1].
\end{align}
Subtracting $\sigma(0)\left(\phi^N_v(\epsilon)-\phi^N_v(0)\right)$ from the first term in \eqref{equation:ansatz} and using \eqref{equation:1}, we get
\begin{align}
	\int_{0}^{\epsilon}\sigma^\prime(0)s \nabla \phi^N_v(s)\mathrm{d}s
\end{align}


==> def_gff.tex <==
We first want to introduce the Gaussian Free Field (GFF) and investigate some of its key properties.
Let $N \in \mathbbm{N}$, $V_N \coloneqq ([0,N]\cap \mathbbm{Z})^2$ of side length $N+1$.


For $B \subseteq V_N$ we write $\mathcal{F}_B \coloneqq \sigma()

==> dgff_results.tex <==
We want to summarize known results for the DGFF, first to see the connection to branching Brownian motion/branching random walk, at least on the level of results, and second, give a taste of what could be possible to prove in the scale-inhomogeneous case. Therefore, recall the notation for the maximum of the DGFF $\phi_N^* \coloneqq \max_{v \in V_N} \phi_v^N.$
In 2001 Bolthausen, Deuschel and Giacomin proved the first order of the maximum:
\begin{thm}[cp. {\cite[Theorem 2]{MR1880237}}]
	For $N\in \mathbbm{N},$ let $\phi^N$ be a discrete GFF on $V_N$. Then,
	\begin{equation}
		\lim_{N \rightarrow \infty} \frac{\phi_N^*}{\log(N^2)} = 1 \quad \text{in probability.}
	\end{equation}
\end{thm}
Let $M_N \coloneqq \phi_N^* - \mathbbm{E}[\phi_N^*]$ be the centred maximum. Bramson and Zeitouni proved in 2011 tightness around the mean and identified the second order.
\begin{thm}[cp. {\cite[Theorem 1.1]{MR2846636}}]
	For $N\in \mathbbm{N}$, let $\phi^N$ be a discrete GFF on $V_N$. Then it holds, that the sequence $\{M_N\}_{N \geq 1}$ is tight.
\end{thm}
The proof of this statement relies on the following \autoref{thm:2ndorderdgff} and similarly to the case of branching random walks, on a Dekking-Host type of argument, which itself uses the strong Markov field property.
In particular, in the same paper the second order correction was explicitly stated:
\begin{thm}\label{thm:2ndorderdgff}
	For $N\in \mathbbm{N},$ let $\phi^N$ be a discrete GFF on $V_N$. It follows, that
	\begin{equation}
		\lim_{N \rightarrow \infty} \frac{\phi_N^* - \log(N^2)}{\log(\log(N))}= - \frac{3}{4} \quad \text{in probability.}
	\end{equation}
	Moreover,
	\begin{equation}
		\mathbbm{E}[\phi_N^*]= 2 \log(N)- \frac{3}{4} \log (\log(N)) +O(1).
	\end{equation}
\end{thm}
The proof relies in comparing the GFF to another Gaussian process of similar covariance structure via an application of Sudakov-Fernique (cf. \autoref{thm:sudakov}). For the auxiliary process one can identify the second order correction via a 2nd moment argument, analogously to the case of branching random walks.
Once established fluctuations of order $O(1)$, it is natural to ask for convergence in law of the centred maximum $\left\{\phi_N^*-\mathbbm{E}\left[\phi_N^*\right]\right\}_{N\in \mathbbm{N}}$, which was then established in 2013 by Bramson, Ding and Zeitouni:
\begin{thm}[cp. {\cite[Theorem 1.1]{MR3433630}}]
	The law of the random variable $M_N= \phi_N^* - \mathbbm{E}[\phi_N^*]$ converges in distribution to a non-degenerate law $\mu_\infty$, as $N \rightarrow \infty$.
	Moreover, there exists a random variable $Z>0$ and a constant $\alpha^* >0$, such that
	\begin{equation}
		\mu_{\infty}((-\infty,x])= \mathbbm{E}[\exp(-\alpha^* Z e^{-2x})].
	\end{equation}
	%(check the constant 2 $\pi$!!! idea: replace it by 2 since guess: $\sqrt{2 \pi}= 2{\sqrt{\frac{\pi}{2}}}$)
\end{thm}
In \cite{MR3509015}, Biskup and Louidor identified first, the random variable $Z$ as a version of the so-called derivative martingale, associated with the continuous GFF.
In the same paper, they discuss varies properties of the so-called "derivative martingale" $Z$.
The constant $\alpha^{*}$ can be explicitely obtained from the right-tail asymptotics of the centered maximum (). The reason for factorizing this constant is due to the fact, that they play substantially different roles in the proof, that is informally $Z$ depends only on the large scales contributions, whereas the constant $alpha^{*}$ depends solely on the small scale increments. Moreover, they have proved the convergence in distribution of a localized version of the extremal process, $\eta_N\coloneqq \sum_{v\in V_N}\delta_{v/N}\otimes \delta_{\phi_v^N-\phi_N^{*}}$, which encodes both the normalised position and height of extremal particles, and identified the limit. Due to heavy correlations nearby local extrema, one expects that clusters of extremal particles form around these, just as in the case of branching Brownian motion (see \cite{2016arXiv160600510B} and \cite{2014arXiv1412.5975B}). Indeed, later in \cite{2016arXiv160600510B} Biskup and Louidor also proved this.
With this, analogous results to the branching Brownian motion have been proved for the discrete GFF.
\begin{rem}
	One should read the results for the GFF, keeping in mind the corresponding results established for the branching random walk, and branching Brownian motion respectively. More precisely, the results resemble each other (cp. \autoref{thm:2nd_order_ibrw}) with the main difference in the scaling in terms of the logarithm (i.e. replace $\log(N)$ just by $n$ with $N=2^n$). The apparent connection is not only true in terms of the results but indeed, it is far deeper.
	Most of the proofs in the above-mentioned papers rely on the construction of various tree or tree-like structures, on which one then defines generalized Gaussian processes resembling branching random walks that approximate the covariance structure of the GFF and which are easier to handle. In the last step, one uses classical Gaussian comparison tools, such as Sudakov-Fernique (\autoref{thm:sudakov}) or Slepian's Lemma (\autoref{thm:slepian}) to reduce the proof of the desired results to a proof of the same results, just for the auxiliary processes, which are easier to achieve, due to their approximate tree structures.
\end{rem}

==> sigma_lambda_dgff_results.tex <==
\begin{comment}
	\begin{figure}
	\begin{tikzpicture}[xscale=2]
	%\draw[xstep=1cm, ystep=1cm, ,color=lightgray] (0,0) grid (4,4);
	
	\draw[->] (-0.25,0)--(4.45,0) node[below]{\footnotesize $\lambda$}; %y axis%
	
	%\foreach \x in {1,...,4}
	%\draw[shift={(\x,0)},color=black] (0pt,2pt) -- (0pt,-2pt) node[below]
	%{\footnotesize $\x$};
	
	\draw[->] (0,-0.25) -- (0,4.5) node[left] {$\color{blue}\mathcal{I}_{\sigma^2}(\lambda)$}; %x axis%
	
	%\foreach \y in {1,...,4}
	%\draw[shift={(0,\y)},color=black] (2pt,0pt) -- (-2pt, 0pt) node[left]
	%{\footnotesize $\y$};
	
	\draw[color=black] (0pt, -5pt) node[below] {\footnotesize $0$};
	
	\draw[color=red] (0,0) -- (4,4) node[midway,above] {\footnotesize $1$};
	%\draw[color=red] (1,2) -- (2,3) node[midway,above] {\footnotesize $\bar{\sigma}_2^2$};
	%\draw[color=red] (2,3) -- (4,4) node[midway,above] {\footnotesize $\bar{\sigma}_3^2$};
	
	\draw[color=blue] (0,0) -- (0.8,0.3) node[midway,below] {\footnotesize $\sigma_1^2$};
	\draw[color=blue] (0.8,0.3) -- (1.3,1) node[midway,below] {\footnotesize $\sigma_2^2$};
	\draw[color=blue] (1.3,1) -- (3.5,1.5) node[midway,below] {\footnotesize $\sigma_3^2$};
	\draw[color=blue] (3.5,1.5) -- (4,4) node[midway,right] {\footnotesize $\sigma_4^2$};
	%\draw[color=blue] (2,3) -- (2.5,3.25) node[midway,below] {\footnotesize $\sigma_5^2$};
	%\draw[color=blue] (2.5,3.25) -- (3.25,3.3) node[midway,below] {\footnotesize $\sigma_6^2$};
	%\draw[color=blue] (3.25,3.3) -- (4,4) node[midway,below] {\footnotesize $\sigma_7^2$}; 
	
	%\draw[color=black] (1,-2pt) node[below] {\footnotesize $\lambda^1$};
	\draw[color=black] (0.8,-3.5pt) node[below] {\footnotesize $\lambda_1$};
	%\draw[color=black] (1.3,-15pt) node[below] {\footnotesize $\lambda_2$};
	\draw[color=black] (1.3,-3.5pt) node[below] {\footnotesize $\lambda_2$};
	%\draw[color=black] (2,-2pt) node[below] {\footnotesize $\lambda^2$};
	%\draw[color=black] (2,-15pt) node[below] {\footnotesize $\lambda_4$};
	%\draw[color=black] (2.5,-3.5pt) node[below] {\footnotesize $\lambda_5$};
	\draw[color=black] (3.5,-3.5pt) node[below] {\footnotesize $\lambda_3$};
	\draw[color=black] (4,-2pt) node[below] {\footnotesize $1=\lambda^1$};
	\draw[color=black] (4,-15pt) node[below] {\footnotesize $\lambda_4$};
	
	\draw[densely dashed,color=gray] (0.8,0.3) -- (0.8,0);
	%\draw[dashed,color=gray] (1.3,2) -- (1.3,0);
	\draw[dashed,color=gray] (1.3,1) -- (1.3,0);
	%\draw[dashed,color=gray] (2,3) -- (2,0);
	%\draw[dashed,color=gray] (2.5,3.25) -- (2.5,0);
	\draw[dashed,color=gray] (3.5,1.3) -- (3.5,0);
	\draw[dashed,color=gray] (4,4) -- (4,0);
	
	\end{tikzpicture}
	\caption{An example of variance.}
	\end{figure}
\end{comment}

